Seeing Invisible Poses: Estimating 3D Body Pose from Egocentric Video

Understanding the camera wearer's activity is central to egocentric vision, yet one key facet of that activity is inherently invisible to the camera--the wearer's body pose. Prior work focuses on estimating the pose of hands and arms when they come into view, but this 1) gives an incomplete view of the full body posture, and 2) prevents any pose estimate at all in many frames, since the hands are only visible in a fraction of daily life activities. We propose to infer the "invisible pose" of a person behind the egocentric camera. Given a single video, our efficient learning-based approach returns the full body 3D joint positions for each frame. Our method exploits cues from the dynamic motion signatures of the surrounding scene--which changes predictably as a function of body pose--as well as static scene structures that reveal the viewpoint (e.g., sitting vs. standing). We further introduce a novel energy minimization scheme to infer the pose sequence. It uses soft predictions of the poses per time instant together with a non-parametric model of human pose dynamics over longer windows. Our method outperforms an array of possible alternatives, including deep learning approaches for direct pose regression from images.

==> noground.tex <==
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c1.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b1.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q1.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c2.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b2.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q2.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c4.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b4.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q4.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c5.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b5.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q5.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c6.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b6.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q6.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c7.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b7.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q7.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c10.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b10.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q10.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c11.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b11.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q11.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c12.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b12.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q12.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c14.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b14.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q14.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c16.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b16.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q16.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c17.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b17.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q17.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c18.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b18.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q18.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c19.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b19.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q19.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c20.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b20.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q20.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c22.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b22.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q22.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c23.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b23.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q23.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c25.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b25.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q25.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c26.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b26.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q26.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c27.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b27.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q27.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c28.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b28.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q28.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c29.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b29.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q29.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c30.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b30.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q30.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c31.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b31.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q31.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c35.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b35.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q35.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c36.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b36.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q36.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c37.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b37.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q37.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c38.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b38.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q38.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c39.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b39.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q39.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c40.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b40.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q40.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c41.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b41.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q41.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c42.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b42.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q42.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c43.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b43.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q43.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c44.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b44.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q44.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c45.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b45.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q45.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c46.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b46.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q46.png}%
\linebreak
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c47.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b47.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q47.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c48.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b48.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q48.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/c49.png}%
\includegraphics[width=0.137859\textwidth,height=0.06\textwidth]{figure/all_example2/res/b49.png}%
\includegraphics[width=0.054282\textwidth,height=0.06\textwidth]{figure/all_example2/res/q49.png}%
\linebreak

